Star Panoptic Quality: Selectively Evaluating Split and Merged Instances

Detecting individual instances is crucial for many segmentation problems. However, expert instance annotations are often unavailable, so instances are approximated heuristically (e.g., as connected components of semantic maps), which can merge touching objects or split fragmented ones. Even when expert annotations exist, expert disagreement or structural delineation biases can yield split or merged reference instances, corresponding to over- or under-segmentation, respectively. Panoptic Quality (PQ) and related metrics capture both segmentation and detection quality while weighting all instances equally, regardless of size. Yet when the references are biased, these metrics can neither detect split or merged instances nor distinguish valid from invalid overor under-segmentation. We present Star Panoptic Quality (StarPQ), a novel evaluation ramework, which closes this gap in two steps: First, we construct a so-called star forest in the bipartite graph whose clean, merge, and split stars isolate different failure modes. Second, we calculate the final metric by individually weighting each failure mode, allowing practitioners to account for instance delineation biases. Across various experiments, we demonstrate that StarPQ not only enables targeted penalization or eniency towards specific failure modes, but also serves as a diagnostic tool to reveal their prevalence.

==> config/commands.tex <==
\definecolor{todo}{RGB}{213,94,0}     %
\definecolor{debug}{RGB}{0,114,178}   %

\makeatletter

\NewDocumentCommand{\todo}{m}{%
  \ifdebug
    \textcolor{todo}{[\textbf{TODO:} #1]}%
  \else
    \@bsphack
    \PackageWarning{commands}{Unresolved TODO in \CurrentFile}%
    \@esphack
  \fi
}

\NewDocumentCommand{\debug}{m}{%
  \ifdebug
    \textcolor{debug}{[#1]}%
  \else
    \@bsphack\@esphack
  \fi
}

\makeatother

\NewDocumentEnvironment{debugblock}{+b}{%
  \ifdebug
    \par\color{debug}%
    \noindent\textbf{[DEBUG]}\par
    #1\par
    \noindent\textbf{[/DEBUG]}\par
  \fi
}{}

\NewDocumentEnvironment{todoblock}{m +b}{%
  \ifdebug
    \par\color{todo}%
    \noindent\textbf{[TODO: #1]}\par
    #2\par
    \noindent\textbf{[/TODO]}\par
  \else
    \PackageWarning{commands}{Unresolved TODO block in \CurrentFile}%
    \par #2\par
  \fi
}{}

\makeatletter
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
  {.1em \@plus1ex \@minus.1ex}%
  {-1em}%
  {\normalfont\normalsize\bfseries}}
\makeatother

\newcommand{\TP}{\text{TP}}
\newcommand{\FP}{\text{FP}}
\newcommand{\FN}{\text{FN}}
\newcommand{\IoU}{\text{IoU}}
\newcommand{\IoL}{\text{IoL}}
\newcommand{\PQ}{\text{PQ}}
\newcommand{\SQ}{\text{SQ}}
\newcommand{\RQ}{\text{RQ}}
\newcommand{\StarPQ}{\text{StarPQ}}

